Tropical optimization technique in bi-objective project scheduling under temporal constraints

We consider a project that consists of a set of activities performed in parallel under constraints on their start and finish times, including start-finish precedence relationships, release start times, release end times, and deadlines. The problems of interest are to decide on the optimal schedule of the activities to minimize both the maximum flow-time over all activities, and the project makespan. We formulate these problems as bi-objective optimization problems in the framework of tropical mathematics which investigates the theory and applications of algebraic systems with idempotent operations and has various applications in management science and operations research. Then, the use of methods and techniques of tropical optimization allows to derive complete Pareto-optimal solutions of the problems in a direct explicit form ready for further analysis and straightforward computation. We discuss the computational complexity of the solution and give illustrative examples.

==> tikzlibraryperspective.code.tex <==
% Copyright 2019 by Max Snippe
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

%\ProvidesFileRCS{tikzlibraryperspective.code.tex}
% Initialize affine transformation matrix for perspective view
% [aa ab ac 0]
% [ba bb bc 0]
% [ca cb cc 0]
% [da db dc 1]
\pgfmathsetmacro\pgf@H@tpp@aa{+1}
  \pgfmathsetmacro\pgf@H@tpp@ab{+0}
    \pgfmathsetmacro\pgf@H@tpp@ac{+0}
\pgfmathsetmacro\pgf@H@tpp@ba{+0}
  \pgfmathsetmacro\pgf@H@tpp@bb{+1}
    \pgfmathsetmacro\pgf@H@tpp@bc{+0}
\pgfmathsetmacro\pgf@H@tpp@ca{+0}
  \pgfmathsetmacro\pgf@H@tpp@cb{+0}
    \pgfmathsetmacro\pgf@H@tpp@cc{+1}
\pgfmathsetmacro\pgf@H@tpp@da{+0}
  \pgfmathsetmacro\pgf@H@tpp@db{+0}
    \pgfmathsetmacro\pgf@H@tpp@dc{+0}

\def\pgfpointperspectivexyz#1#2#3{%
  \pgfmathsetmacro\pgf@pp@w%
    { \pgf@H@tpp@da*(#1) + \pgf@H@tpp@db*(#2) + \pgf@H@tpp@dc*(#3) + 1}
  \pgfmathsetmacro\pgf@pp@x%
    {(\pgf@H@tpp@aa*(#1) + \pgf@H@tpp@ab*(#2) + \pgf@H@tpp@ac*(#3))/\pgf@pp@w}
  \pgfmathsetmacro\pgf@pp@y%
    {(\pgf@H@tpp@ba*(#1) + \pgf@H@tpp@bb*(#2) + \pgf@H@tpp@bc*(#3))/\pgf@pp@w}
  \pgfmathsetmacro\pgf@pp@z%
    {(\pgf@H@tpp@ca*(#1) + \pgf@H@tpp@cb*(#2) + \pgf@H@tpp@cc*(#3))/\pgf@pp@w}
%
  \pgf@x=\pgf@pp@x\pgf@xx%
  \advance\pgf@x by \pgf@pp@y\pgf@yx%
  \advance\pgf@x by \pgf@pp@z\pgf@zx%
  \pgf@y=\pgf@pp@x\pgf@xy%
  \advance\pgf@y by \pgf@pp@y\pgf@yy%
  \advance\pgf@y by \pgf@pp@z\pgf@zy}

\tikzdeclarecoordinatesystem{three point perspective}
{%
  \tikzset{cs/.cd,x=0,y=0,z=0,#1}%
  \pgfpointperspectivexyz{\tikz@cs@x}{\tikz@cs@y}{\tikz@cs@z}
}
\tikzaliascoordinatesystem{tpp}{three point perspective}

\pgfkeys{
  /perspective/.cd,
    p/.code args={(#1,#2,#3)}{
      \pgfmathparse{ifthenelse(#1,int(1),int(0))}
      \ifnum\pgfmathresult=0\else
        \pgfmathsetmacro\pgf@H@tpp@ba{#2/#1}
        \pgfmathsetmacro\pgf@H@tpp@ca{#3/#1}
        \pgfmathsetmacro\pgf@H@tpp@da{ 1/#1}
      \fi
    },
    q/.code args={(#1,#2,#3)}{
      \pgfmathparse{ifthenelse(#2,int(1),int(0))}
      \ifnum\pgfmathresult=0\else
        \pgfmathsetmacro\pgf@H@tpp@ab{#1/#2}
        \pgfmathsetmacro\pgf@H@tpp@cb{#3/#2}
        \pgfmathsetmacro\pgf@H@tpp@db{ 1/#2}
      \fi
    },
    r/.code args={(#1,#2,#3)}{
      \pgfmathparse{ifthenelse(#3,int(1),int(0))}
      \ifnum\pgfmathresult=0\else
        \pgfmathsetmacro\pgf@H@tpp@ac{#1/#3}
        \pgfmathsetmacro\pgf@H@tpp@bc{#2/#3}
        \pgfmathsetmacro\pgf@H@tpp@dc{ 1/#3}
      \fi
    },
}

\tikzset{
  perspective/.append code={\pgfkeys{/perspective/.cd,#1}},
  perspective/.default={
    p={(10,0,0)},
    q={(0,10,0)},
    r={(0,0,20)}},
}

\tikzset{
  3d view/.code 2 args={
    % Set elevation and azimuth angles
    \pgfmathsetmacro\pgf@view@az{#1}
    \pgfmathsetmacro\pgf@view@el{#2}
    % Calculate projections of rotation matrix
    \pgfmathsetmacro\pgf@xvec@x{cos(\pgf@view@az)}
    \pgfmathsetmacro\pgf@xvec@y{-sin(\pgf@view@az)*sin(\pgf@view@el)}
    \pgfmathsetmacro\pgf@yvec@x{sin(\pgf@view@az)}
    \pgfmathsetmacro\pgf@yvec@y{cos(\pgf@view@az)*sin(\pgf@view@el)}
    \pgfmathsetmacro\pgf@zvec@x{+0}
    \pgfmathsetmacro\pgf@zvec@y{cos(\pgf@view@el)}
    % Set base vectors
    \pgfsetxvec{\pgfpoint{\pgf@xvec@x cm}{\pgf@xvec@y cm}}
    \pgfsetyvec{\pgfpoint{\pgf@yvec@x cm}{\pgf@yvec@y cm}}
    \pgfsetzvec{\pgfpoint{\pgf@zvec@x cm}{\pgf@zvec@y cm}}
  },
  3d view/.default={-30}{15},
  isometric view/.style={3d view={-45}{atan(1/sqrt(2))}},
}

\endinput

